Learning a Hierarchical Planner from Humans in Multiple Generations

A typical way in which a machine acquires knowledge from humans is by programming. Compared to learning from demonstrations or experiences, programmatic learning allows the machine to acquire a novel skill as soon as the program is written, and, by building a library of programs, a machine can quickly learn how to perform complex tasks. However, as programs often take their execution contexts for granted, they are brittle when the contexts change, making it difficult to adapt complex programs to new contexts. We present natural programming, a library learning system that combines programmatic learning with a hierarchical planner. Natural programming maintains a library of decompositions, consisting of a goal, a linguistic description of how this goal decompose into sub-goals, and a concrete instance of its decomposition into sub-goals. A user teaches the system via curriculum building, by identifying a challenging yet not impossible goal along with linguistic hints on how this goal may be decomposed into sub-goals. The system solves for the goal via hierarchical planning, using the linguistic hints to guide its probability distribution in proposing the right plans. The system learns from this interaction by adding newly found decompositions in the successful search into its library. Simulated studies and a human experiment (n=360) on a controlled environment demonstrate that natural programming can robustly compose programs learned from different users and contexts, adapting faster and solving more complex tasks when compared to programmatic baselines.

==> sections/np_search_alg.tex <==
\begin{algorithm}
\begin{algorithmic}
\label{alg:dfs}
\Function{NP}{$q$, $s_0$, $\M(c)$}
\State $S \gets$ \Call{Stack}{ }
\State \Call{Push}{$S$, $\langle s_0, [q], q.goal \rangle$}

\While{$S$ is not empty}
    \State $x \gets$ \Call{Pop}{$S$}
    \State $x' \gets$ \Call{PrefixExecution}{$q_{seq}$, $s$, $\M(c)$} \Comment{execute all prefix actions, update states}

    \If{$x'$ is error}
        \State \textbf{continue} \Comment{crashes or fails first goal, discard}
        
    \ElsIf{$x$ is $\langle s, q_{seq}, g \rangle$} \Comment{of the form state, sequence of search problems, and final goal}
        \State $decomposed \gets$ \Call{propose}{$q'$, $\LL$, n\_times} \Comment{decompose into other search problems}
        
        \For{$[\textit{np}_1^i, \ldots, \textit{np}_n^i]_i \in decomposed$}
            \State $np_\text{expnd} \gets \textit{np}[\textit{np}' := \textit{np}': [\textit{np}_1^i, \ldots, \textit{np}_n^i]]$ \Comment{Expand $\textit{np'}$ with the decomposition}
            \State \Call{Push}{$S$, $\langle \textit{np}_\text{expnd}, s' \rangle$}
        \EndFor

    \Else
        \State \textbf{return} $\textit{np}$ \Comment{It must be that $\textit{np}$ is a concrete program that satisfies all constraints}
    \EndIf
\EndWhile

\EndFunction
\end{algorithmic}
\caption{Natural Programming Execution}
\end{algorithm}
